Convergent Graph Solvers

We propose the convergent graph solver (CGS), a deep learning method that learns iterative mappings to predict the properties of a graph system at its stationary state (fixed point) with guaranteed convergence. CGS systematically computes the fixed points of a target graph system and decodes them to estimate the stationary properties of the system without the prior knowledge of existing solvers or intermediate solutions. The forward propagation of CGS proceeds in three steps: (1) constructing the input dependent linear contracting iterative maps, (2) computing the fixed-points of the linear maps, and (3) decoding the fixed-points to estimate the properties. The contractivity of the constructed linear maps guarantees the existence and uniqueness of the fixed points following the Banach fixed point theorem. To train CGS efficiently, we also derive a tractable analytical expression for its gradient by leveraging the implicit function theorem. We evaluate the performance of CGS by applying it to various network-analytic and graph benchmark problems. The results indicate that CGS has competitive capabilities for predicting the stationary properties of graph systems, irrespective of whether the target systems are linear or non-linear. CGS also shows high performance for graph classification problems where the existence or the meaning of a fixed point is hard to be clearly defined, which highlights the potential of CGS as a general graph neural network architecture.

==> sections/1-introduction.tex <==
Our world is replete with networked systems, where their overall properties emerge from complex interactions among the system entities. Such networked systems attain their unique properties from their stationary states and hence, finding these stationary properties is a common goal for many problems that arise in the science and engineering field. Examples of such problems include the minimization of the molecule's potential energy that finds the stationary positions of the atoms to compute the potential energy of the molecule \citep{moloi2005iterative}, the PageRank algorithm that finds the stationary importance of online web pages to compute recommendation scores \citep{brin1998anatomy}, and the network analysis of fluid flow in porous media that finds the stationary pressures in pore networks to compute the macroscopic properties of the media \citep{gostick2016openpnm}.

% The iterative methods typically derive an analytic iterative map to compute the updated states from the previous state based on the knowledge of the target problem. 

In these network-analytic problems, the network is often represented as a graph, and the stationary states are often computed through problem-specific iterative methods. These iterative methods typically derive an analytic iterative map based on a priori knowledge of the target problem. By applying the iterative map repeatedly, these methods compute the stationary states (fixed points) and the associated properties of the target system.

Instead of designing the problem-specific iterative methods, researchers have suggested to employ deep learning approaches to \textit{learn} the iterative methods. Such approaches can be classified into two classes: \textit{hybrid} and \textit{native} approaches. Hybrid approaches combine an existing iterative method with a feed-forward network to compute the properties of the target system accurately while enhancing the convergence property and the solution quality of the existing method \citep{hsieh2019learning, huang2020int, poli2020hypersolvers}. Native approaches employ learnable iterative methods that do not require any existing iterative methods. For the native approaches, the initial states are either constant or learned values, the iterative maps are learned using graph neural networks (GNNs), and the learned iterative maps are applied to find the fixed points \citep{scarselli2008graph, dai2018learning, liao2018reviving, gu2020implicit}.

%Finding Gaps in the previous research
Despite being able to learn the iterative maps, the aforementioned approaches entail challenges. To promote the convergence properties of the learned solvers, knowledge of the analytic iterative map is required for the hybrid approaches to compute the fixed points or intermediate states. However, satisfying this requirement is often difficult for complex target systems. On the other hand, the existence of the fixed points of the learned iterative maps is seldom guaranteed by the native approaches. As a result, the number of iterative steps is needed to be prescribed as a hyperparameter to ensure the termination of the iterations, which may cause premature termination or inefficient backward propagation if the iteration number is inadequately small or too large respectively. 

% Furthermore, as the iterative step increases, both the hybrid and native approaches may encounter the problems of slow forward propagation and vanishing gradient. 

%Formulation perspective: 문제를 어떻게 formulation했는지를 기술하고 그를 통해 얻을 수있는 장점. CGS가 어떻게 문제를 푸는 지 high-level에서 기술
% In this study, we propose the convergent graph solver (CGS), a deep learning method that learns iterative mappings to predict the properties of a graph system at its stationary states (fixed points) with guaranteed convergence. CGS systematically computes the fixed points of a target graph system and decodes them to estimate the system's stationary properties without requiring the prior knowledge of existing solvers and intermediate solutions.
% %Computation perspective: 무엇을 했는지와 그것으로 야기되는 장점을 tight하게 연결하여 기술
% To overcome the aforementioned challenges of existing learning-based iterative approaches, the forward propagation of CGS is designed to proceed in the following three steps:

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Constructing linear contracting iterative maps}: CGS uses the input graph, which dictates the specification of the target network-analytic problems, to construct a set of linear contracting maps, where each of which is guaranteed to have an unique fixed point.
%     \item \textbf{Computing fixed-point via iterative methods}: CGS computes the solution of constructed linear maps via iterative methods and then compute the corresponding gradients via the implicit function theorem. This design choice allows CGS to backpropagate with $\mathcal{O}(1)$ memory consumption over the iterative steps.
%     \item \textbf{Decoding fixed-points to estimate the properties}: CGS decodes the computed fixed points to estimate the properties of the target system. 
% \end{itemize}


In this study, we propose the convergent graph solver (CGS), a deep learning method that learns to construct iterative mappings that predict the properties of a graph system at its stationary states (fixed points) with \textit{guaranteed convergence}. CGS computes the fixed points of a target graph system and decodes them to estimate the system's stationary properties without requiring the prior knowledge of existing solvers and intermediate solutions. The forward propagation of CGS is designed to proceed in the following three steps: (1) constructing the input-dependent linear-contracting iterative maps from the input graph via encoder networks, (2) computing the fixed points via iterative methods, and (3) decoding the fixed points to estimate the properties. This learning to generate the iterative maps from the inputs strategy is simple but flexible design as we do not make any structural assumptions on the encoder network, unlike the previous methods \cite{gu2020implicit, tiezzi2020lagrangian}. Furthermore, we employ an implicit function theorem that enables $\mathcal{O}(1)$ memory consumption over the iterative steps to train CGS efficiently.

% The unique novelties of CGS are as follows:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Input dependent linear contracting iterative maps}: CGS uses the input graph, which dictates the specification of the target network-analytic problem, to construct a set of linear contracting maps, each of which is guaranteed to have the unique fixed point that embeds the important features for conducting various end tasks.
%     \item \textbf{Fixed point based forward and backward computation}: CGS computes the solution of constructed linear maps via iterative methods (or direct inversion) and use them to (2) compute efficiently the gradient via the implicit function theorem during training phase ($\mathcal{O}(1)$ memory consumption over the iterative steps), or (2) predict the output with the imposed behavioral inductive biases during execution phase.
% \end{itemize}

%Application perspective
We evaluate the performance of CGS using two types of paradigmatic network-analytic problems: physical diffusion in networks and the Markov decision process, where the true labels can be computed analytically using linear and non-linear analytical iterative methods respectively. We also employ CGS to solve various graph classification benchmark tasks. The results show that the prediction accuracy of CGS is on-par or superior to that of deep graph models, and suggest that CGS can be an effective general computational layer for processing graph-structured data.




==> tables/rebuttal.tex <==
\begin{table}[t]
\caption{\textbf{Stochastic GVI}}
\label{table:SGVI}
\centering


\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|c}
\toprule
$n_s$ & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{50} & \multicolumn{2}{c}{75} & \multicolumn{2}{c}{100} & \#. params \\
\midrule
$n_a$ & 5 & 10 & 10 & 15 & 10 & 15 & 10 & 15 & \\
\midrule
{\fontfamily{lmtt}\selectfont SSE} & 
\begin{tabular}[c]{@{}c@{}} 7.74 $\pm$ 4.61 \\ (0.73 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 14.06 $\pm$ 3.59 \\ (0.77 $\pm$ 0.10 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 13.65 $\pm$ 2.19 \\ (0.77 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 98.97 $\pm$ 0.03 \\ (0.22 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 13.71 $\pm$ 1.82 \\ (0.76 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 98.97 $\pm$ 0.02 \\ (0.18 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 13.69 $\pm$ 1.57 \\ (0.76 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 98.97 $\pm$ 0.01 \\ (0.17 $\pm$ 0.05 \%) \end{tabular} &
43,521 \\
{\fontfamily{lmtt}\selectfont IGNN} & 
\begin{tabular}[c]{@{}c@{}} 12.72 $\pm$ 4.97 \\ (0.79 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 35.34 $\pm$ 1.43 \\ (0.77 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 34.95 $\pm$ 0.90 \\ (0.76 $\pm$ 0.07 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 46.02 $\pm$ 1.19 \\ (0.82 $\pm$ 0.10 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 34.93 $\pm$ 0.71 \\ (0.76 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 45.64 $\pm$ 0.66 \\ (0.80 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 34.86 $\pm$ 0.65 \\ (0.75 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 45.61 $\pm$ 0.55 \\ (0.79 $\pm$ 0.05 \%) \end{tabular} &
268,006 \\
{\fontfamily{lmtt}\selectfont CGS(16)} &
\begin{tabular}[c]{@{}c@{}} 2.92 $\pm$ 1.71 \\ (0.70 $\pm$ 0.12 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.13 $\pm$ 0.78 \\ (0.71 $\pm$ 0.12 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 0.93 $\pm$ 0.48 \\ (0.71 $\pm$ 0.07 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.01 $\pm$ 0.57 \\ (0.74 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 0.84 $\pm$ 0.35 \\ (0.71 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.00 $\pm$ 0.33 \\ (0.74 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 0.81 $\pm$ 0.29 \\ (0.71 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 0.96 $\pm$ 0.29 \\ (0.74 $\pm$ 0.05 \%) \end{tabular} &
258,485 \\
{\fontfamily{lmtt}\selectfont CGS(32)} &
\begin{tabular}[c]{@{}c@{}} 3.32 $\pm$ 2.09 \\ (0.70 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.91 $\pm$ 1.10 \\ (0.69 $\pm$ 0.12 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.25 $\pm$ 0.61 \\ (0.70 $\pm$ 0.07 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 3.08 $\pm$ 0.89 \\ (0.70 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.16 $\pm$ 0.52 \\ (0.70 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.52 $\pm$ 0.41 \\ (0.71 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.13 $\pm$ 0.46 \\ (0.70 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.37 $\pm$ 0.36 \\ (0.70 $\pm$ 0.05 \%) \end{tabular} &
265,701 \\
{\fontfamily{lmtt}\selectfont CGS(64)} &
\begin{tabular}[c]{@{}c@{}} 4.18 $\pm$ 2.62 \\ (0.70 $\pm$ 0.12 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 2.02 $\pm$ 1.00 \\ (0.71 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.87 $\pm$ 0.66 \\ (0.71 $\pm$ 0.07 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.23 $\pm$ 0.57 \\ (0.73 $\pm$ 0.11 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.86 $\pm$ 0.58 \\ (0.71 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.39 $\pm$ 0.37 \\ (0.72 $\pm$ 0.06 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.83 $\pm$ 0.54 \\ (0.71 $\pm$ 0.05 \%) \end{tabular} &
\begin{tabular}[c]{@{}c@{}} 1.40 $\pm$ 0.33 \\ (0.72 $\pm$ 0.05 \%) \end{tabular} &
280,133 \\

\bottomrule
\end{tabular}
}
\end{table}
